VGGT: Visual Geometry Grounded Transformer

We present VGGT, a feed-forward neural network that directly infers all key 3D attributes of a scene, including camera parameters, point maps, depth maps, and 3D point tracks, from one, a few, or hundreds of its views. This approach is a step forward in 3D computer vision, where models have typically been constrained to and specialized for single tasks. It is also simple and efficient, reconstructing images in under one second, and still outperforming alternatives that require post-processing with visual geometry optimization techniques. The network achieves state-of-the-art results in multiple 3D tasks, including camera parameter estimation, multi-view depth estimation, dense point cloud reconstruction, and 3D point tracking. We also show that using pretrained VGGT as a feature backbone significantly enhances downstream tasks, such as non-rigid point tracking and feed-forward novel view synthesis. Code and models are publicly available at https://github.com/facebookresearch/vggt.

==> figures/fig_transformer_architecture_types.tex <==
\begin{figure}
\centering
% \vspace{3cm}
% \TODO{Comparison between encoder-decoder, decoder-only, and attention-alternating architectures.}
% \vspace{3cm}
\includegraphics[width=\linewidth]{figures/transformer_comparison.pdf}
\caption{
Comparison between transformer architectures for multi-view dense prediction.
(a) encoder-decoder used by DUSt3r \cite{wang24dust3r:}, LRM \cite{hong24lrm:},
(b) decoder-only used by LVSM \cite{jin24lvsm:}, MeshLRM \cite{wei24meshlrm:},
(c) our Attention-Alternating (AA). \TODO{Remove or modify this Figure. We need to highlight the difference between self att only and self att + cross att}
% \jianyuan{Simple one for SRT. Will replace the grey tokens by real images. }
}%
\label{fig:transformer_architecture_types}
\end{figure}

==> tables/point_nvs.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Measuring Point Cloud Quality by Novel View Synthesis}. Comparing point clouds in different coordinates are always hard. It is reasonable to align different point clouds by ICP, but such alignment is very sensitive to hyperparameter setting. While at the same time, recent methods have per pixel point maps and their aligned camera poses.  In this case, we can measure the quality of point cloud by fitting a 3D gaussian model with the xyz of gaussians fixed. To avoid the effect of inaccurate poses, we use the methods' own camera poses as initilization and keep them optimized during gaussian fitting. 
\label{tab:nvs_pcl}
\jianyuan{I will remove this from caption and put it in the exp section. }
% Instead of directly comparing point cloud,.
}
\begin{tabular}{c|c|c}
% \hline
PSNR & Co3D & DL3DV \\ \hline
Dust3R & &  \\ \hline
Mast3R &  &  \\ \hline
Ours &  &  \\ 
\hline
\end{tabular}
\end{table}











